RunyaNER: Auxiliary Language Selection for Runyankore NER

Cross-lingual zero-shot transfer and multilingual fine-tuning are promising approaches for NLP tasks such as Named Entity Recognition (NER) in low-resource languages, but in the absence of target language benchmarks, it is unclear which auxiliary language selection strategy leads to the best transfer. We introduce RunyaNER, the first publicly available NER benchmark for the East African language Runyankore, and use it to investigate the choice of which languages to use for transfer. Created with a semi-automated pipeline and fully manually verified, RunyaNER contains over 237k annotated words across 30k sentences. We benchmark pretrained models on RunyaNER, establishing that our dataset is of sufficient quality and size to produce effective Runyankore NER models. We then use RunyaNER to investigate auxiliary language selection in cross-lingual zero-shot and multilingual fine-tuning settings. Our experiments show that while transfer performance is highly sensitive to auxiliary language selection, embedding-based measures computed from labelled training spans correlate more strongly with downstream transfer performance than traditional linguistic features based on metadata or typology. By releasing RunyaNER and providing a systematic analysis of auxiliary language selection strategies, this work contributes both a new benchmark resource and practical insights for multilingual transfer in low-resource settings.

==> diagrams/cosine_diagram.tex <==
\begin{tikzpicture}[
    >=Latex,
    box/.style={rectangle, rounded corners, draw, align=center, minimum width=34mm, minimum height=11mm},
    tinybox/.style={rectangle, draw, minimum width=8mm, minimum height=7mm, inner sep=0pt, font=\scriptsize},
    groupbox/.style={rounded corners, draw, inner sep=4mm},
    label/.style={font=\small, align=center}
]
% -----------------------------
% Row 1: BIO-annotated corpora
% -----------------------------
\node[box, fill=blue!10] (bioRNY) {BIO-annotated\\Runyankore \\ (RunyaNER)};
\node[box, fill=blue!10, right=25mm of bioRNY] (bioL2) {BIO-annotated\\Aux Lang 2\\ (MasakhaNER)};
\node[box, fill=blue!10, right=25mm of bioL2] (bioL3) {BIO-annotated\\Aux Lang 3\\(MasakhaNER)};

% -----------------------------
% Row 2: PLM embeddings
% -----------------------------
\node[box, fill=green!10, below=22mm of bioRNY] (plmRNY) {PLM encoder\\(layer-wise embeddings)};
\node[box, fill=green!10, below=22mm of bioL2] (plmL2) {PLM encoder\\(layer-wise embeddings)};
\node[box, fill=green!10, below=22mm of bioL3] (plmL3) {PLM encoder\\(layer-wise embeddings)};

\draw[->, thick] (bioRNY) -- (plmRNY);
\draw[->, thick] (bioL2) -- (plmL2);
\draw[->, thick] (bioL3) -- (plmL3);

% -----------------------------
% Row 3: Prototypes
% -----------------------------
\coordinate (cRNY) at ($(plmRNY.south)+(0,-28mm)$);
\node[tinybox, fill=yellow!20] (rnyPER)  at ($(cRNY)+(-12mm,  5mm)$) {PER};
\node[tinybox, fill=yellow!20] (rnyORG)  at ($(cRNY)+( 12mm,  5mm)$) {ORG};
\node[tinybox, fill=yellow!20] (rnyLOC)  at ($(cRNY)+(-12mm, -5mm)$) {LOC};
\node[tinybox, fill=yellow!20] (rnyDATE) at ($(cRNY)+( 12mm, -5mm)$) {DATE};
\node[groupbox, fit=(rnyPER)(rnyORG)(rnyLOC)(rnyDATE),
      label={[label]above:{\textbf{Runyankore prototypes}\\(per entity, per layer)}}] (grpRNY) {};

\coordinate (cL2) at ($(plmL2.south)+(0,-28mm)$);
\node[tinybox, fill=yellow!20] (l2PER)  at ($(cL2)+(-12mm,  5mm)$) {PER};
\node[tinybox, fill=yellow!20] (l2ORG)  at ($(cL2)+( 12mm,  5mm)$) {ORG};
\node[tinybox, fill=yellow!20] (l2LOC)  at ($(cL2)+(-12mm, -5mm)$) {LOC};
\node[tinybox, fill=yellow!20] (l2DATE) at ($(cL2)+( 12mm, -5mm)$) {DATE};
\node[groupbox, fit=(l2PER)(l2ORG)(l2LOC)(l2DATE),
      label={[label]above:{\textbf{L2 prototypes}\\(per entity, per layer)}}] (grpL2) {};

\coordinate (cL3) at ($(plmL3.south)+(0,-28mm)$);
\node[tinybox, fill=yellow!20] (l3PER)  at ($(cL3)+(-12mm,  5mm)$) {PER};
\node[tinybox, fill=yellow!20] (l3ORG)  at ($(cL3)+( 12mm,  5mm)$) {ORG};
\node[tinybox, fill=yellow!20] (l3LOC)  at ($(cL3)+(-12mm, -5mm)$) {LOC};
\node[tinybox, fill=yellow!20] (l3DATE) at ($(cL3)+( 12mm, -5mm)$) {DATE};
\node[groupbox, fit=(l3PER)(l3ORG)(l3LOC)(l3DATE),
      label={[label]above:{\textbf{L3 prototypes}\\(per entity, per layer)}}] (grpL3) {};

\draw[->, thick] (plmRNY.south) -- (grpRNY.north);
\draw[->, thick] (plmL2.south) -- (grpL2.north);
\draw[->, thick] (plmL3.south) -- (grpL3.north);

% -----------------------------
% Similarity matrix BELOW (centered under L2/L3)
% -----------------------------
\coordinate (midL2L3) at ($(grpL2.south)!0.5!(grpL3.south)$);

\node[rectangle, rounded corners, draw, minimum width=56mm, minimum height=66mm,
      below=26mm of midL2L3] (simFrame) {};

\foreach \i in {0,...,3} {
  \foreach \j in {0,...,3} {
    \node[tinybox, fill=red!\the\numexpr 20+18*\i\relax,
          minimum width=8mm, minimum height=7mm]
      at ($(simFrame.west)+(14mm + \j*8mm, 22mm - \i*12mm)$) {};
  }
}

\node[anchor=east, font=\scriptsize] at ($(simFrame.west)+(7mm,  22mm)$) {PER};
\node[anchor=east, font=\scriptsize] at ($(simFrame.west)+(7mm,  10mm)$) {ORG};
\node[anchor=east, font=\scriptsize] at ($(simFrame.west)+(7mm,  -2mm)$) {LOC};
\node[anchor=east, font=\scriptsize] at ($(simFrame.west)+(7mm, -14mm)$) {DATE};

\node[anchor=south, font=\scriptsize, rotate=90]
  at ($(simFrame.north west)+(14mm,-2mm)$) {$L_1$};
\node[anchor=south, font=\scriptsize, rotate=90]
  at ($(simFrame.north west)+(22mm,-2mm)$) {$L_2$};
\node[anchor=south, font=\scriptsize, rotate=90]
  at ($(simFrame.north west)+(30mm,-2mm)$) {$\dots$};
\node[anchor=south, font=\scriptsize, rotate=90]
  at ($(simFrame.north west)+(38mm,-2mm)$) {$L_m$};

\draw[->, thick]
  (grpL2.south) -- ($(simFrame.north west)+(10mm,-1mm)$)
  node[pos=0.25, above left=0.7mm and 1mm, fill=white, inner sep=1pt, font=\scriptsize]
    {cosine$(\cdot,\cdot)$};

\draw[->, thick]
  (grpL3.south) -- ($(simFrame.north east)+(-10mm,-1mm)$)
  node[pos=0.25, above right=0.7mm and 1mm, fill=white, inner sep=1pt, font=\scriptsize]
    {cosine$(\cdot,\cdot)$};

\draw[dashed, thick]
  (grpRNY.south) -- (simFrame.north)
  node[pos=0.3, right, fill=white, inner sep=1pt, font=\scriptsize]
    {reference prototypes};

\node[rectangle, draw, fill=white, inner sep=2pt,
      label, anchor=south] (simLabel)
  at ($(simFrame.north)+(0,4mm)$)
  {\textbf{Cosine similarity matrix}\\(auxiliary $\rightarrow$ Runyankore; per layer $\ell$)};

\node[font=\scriptsize, align=left, text width=54mm, anchor=north west]
  at ($(simFrame.south west)+(0pt,-2mm)$)
  {Computed independently for each PLM layer $\ell$; cells encode cosine similarity between auxiliary and Runyankore entity prototypes (PER/ORG/LOC/DATE), for layers $L_1,\dots,L_m$.};

\end{tikzpicture}

==> diagrams/swd_diagram.tex <==
\begin{tikzpicture}[
    >=Latex,
    box/.style={rectangle, rounded corners, draw, align=center, minimum width=38mm, minimum height=11mm, text width=42mm},
    smallbox/.style={rectangle, rounded corners, draw, align=center, minimum width=36mm, minimum height=11mm, font=\scriptsize, text width=46mm},
    label/.style={font=\small, align=center}
]

\node[box, fill=blue!10] (run)
  {BIO-annotated Runyankore corpus\\(RunyaNER)};
\node[box, fill=blue!10, right=40mm of run] (aux)
  {BIO-annotated auxiliary corpus\\(MasakhaNER)};

\node[box, fill=green!10, below=18mm of run] (encR)
  {PLM encoder (all layers)\\tokenization + contextual embeddings};
\node[box, fill=green!10, below=18mm of aux] (encA)
  {PLM encoder (all layers)\\tokenization + contextual embeddings};

\draw[->, thick] (run) -- (encR)
  node[midway, left, xshift=-1mm, fill=white, inner sep=1pt, font=\scriptsize]
    {PLM encoding};
\draw[->, thick] (aux) -- (encA)
  node[midway, right, xshift=1mm, fill=white, inner sep=1pt, font=\scriptsize]
    {PLM encoding};

\node[smallbox, fill=yellow!15, below=16mm of encR] (distR)
  {Span embeddings per entity tag\\(unit-normalized; sampled subset)};
\node[smallbox, fill=yellow!15, below=16mm of encA] (distA)
  {Span embeddings per entity tag\\(unit-normalized; sampled subset)};

\draw[->, thick] (encR) -- (distR)
  node[midway, left, xshift=-1mm, fill=white, inner sep=1pt, font=\scriptsize]
    {extract spans};
\draw[->, thick] (encA) -- (distA)
  node[midway, right, xshift=1mm, fill=white, inner sep=1pt, font=\scriptsize]
    {extract spans};

\coordinate (fanR) at ($(distR.south)+(0,-5mm)$);
\coordinate (fanA) at ($(distA.south)+(0,-5mm)$);
\draw[->, thick] (distR.south) -- (fanR);
\draw[->, thick] (distA.south) -- (fanA);

\node[smallbox, fill=purple!15,
      below=22mm of $(distR.south)!0.5!(distA.south)$] (swd)
  {Sliced Wasserstein Distance (per tag, per layer)\\
   random 1-D projections of span distributions\\
   1-D Wasserstein-1 ($W_1$) distances\\
   average over projection directions};

\draw[->, thick, shorten >=2pt]
  (fanR)
  to[out=-100, in=120, looseness=1.05]
  node[pos=0.45, left, xshift=-1mm, fill=white, inner sep=1pt, font=\scriptsize]
    {Runyankore tag-wise distributions}
  (swd.north west);

\draw[->, thick, shorten >=2pt]
  (fanA)
  to[out=-80, in=60, looseness=1.05]
  node[pos=0.45, right, xshift=1mm, fill=white, inner sep=1pt, font=\scriptsize]
    {Auxiliary tag-wise distributions}
  (swd.north east);

\node[smallbox, fill=gray!10, below=18mm of swd] (agg)
  {Aggregate over entity tags\\
   (mean of tagwise SWD values)\\
   $\Rightarrow$ per-layer SWD score};

\draw[->, thick] (swd.south) -- (agg.north)
  node[midway, right, xshift=1mm, fill=white, inner sep=1pt, font=\scriptsize]
    {average over tags};

\end{tikzpicture}
